Information Complexity and Estimation

We consider an input $x$ generated by an unknown stationary ergodic source $X$ that enters a signal processing system $J$, resulting in $w=J(x)$. We observe $w$ through a noisy channel, $y=z(w)$; our goal is to estimate x from $y$, $J$, and knowledge of $f_{Y|W}$. This is universal estimation, because $f_X$ is unknown. We provide a formulation that describes a trade-off between information complexity and noise. Initial theoretical, algorithmic, and experimental evidence is presented in support of our approach.

==> CNXCS_macros.tex <==
\newcommand{\eps}{\epsilon}
\def\hatomega{ {\widehat{\Omega}} } % index set
\def \real { \mathbb{R} }
\def \A { \mathbb{A} }
\def\hatgamma{ {\widehat{\Gamma}} } % index set
\def \x {x} %{\mathbf{x}} % Signal vector
\def \y {y} % {\mathbf{y}} % Measurements vector
\def \n {n} %{\mathbf{n}} % Noise vector
\def \s {s} %{\mathbf{s}} % Matched filter
\def \MSE {\textrm{MSE}} % Mean Square Error
\newcommand{ \bomega}{\mbox{\boldmath$\omega$}}
\newcommand{ \btheta}{\mbox{\boldmath$\theta$}}
\newcommand{ \balpha}{\mbox{\boldmath$\alpha$}}

\def \m {m} % Measurement index
\def \n {n} % Signal time series index
\def \N {\mathcal{N}} % Signal length
\def \M {M} % Measurement vector length
\def \K {K} % Signal sparsity
\def \C {\mathrm{C}}
\def \trans {^T} % Symbol for transpose: usage \Phi\trans

\def \manifold { \mathcal{M} } % Manifold
\def \condition { \tau } % Niyogi's condition number
\def \regularity { R } % Covering regularity
\def \volume { V } % Manifold volume

\def \thetahat
\def \thresh {{\mathcal{T}}}
\def \thetahat {\widehat{\theta}}
\def \r {{\bf r}}
\def \b {{\bf b}}
\def \e {{\bf e}}
\def \pinv {^\dag}
\def \xhat {\widehat{x}}
\def \zhat {\widehat{z}}
\def \xbar {\bar{x}}
\def \atilde {\widetilde{\alpha}}
\def \alphabet {\mathcal{X}}

\def \Hhat {\widehat{H}}
\def \prob {\mathbb{P}}
\def \Phihat {\widetilde{\Phi}}
\def \Rhat {\widetilde{R}}
\def \bigo {\mathcal{O}}
\def \Hhat {\widetilde{H}}

\def \manifold { \mathcal{M} } % Manifold
\def \condition { \tau } % Niyogi's condition number
\def \regularity { R } % Covering regularity
\def \volume { V } % Manifold volume
\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\dist}[2]{\left\| #1 - #2 \right\|_2}
\newcommand{\norm}[1]{\left\| #1 \right\|_2}
\newcommand{\normsq}[1]{\left\| #1 \right\|_2^2}
\newcommand{\compaction}[3]{(1 - #3)\sqrt{\pdim/\dim} \dist{#1}{#2} \le \dist{\proj#1}{\proj#2} \le (1 +
#3)\sqrt{\pdim/\dim} \dist{#1}{#2}}
\newcommand{\compactionB}[3]{(1 - #3)#2 \le #1 \le (1 +
#3)#2}

\newcommand{\bone}{{\bf1}}
\newcommand{\cl}[1]{{\mathcal{#1}}}
\newcommand{\Eq}{{\mathbb{E}_q}}
\newcommand{\E}{{\mathbb{E}}}
\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\opt}{{\mathrm{opt}}}
\newcommand{\vzero}{{\mathbf{0}}}
\newcommand{\gradnt}{{\nabla}}
\newcommand{\sign}{{\mathrm{sign}}}


